Efficient Ab-Initio Molecular Dynamic Simulations by Offloading Fast Fourier Transformations to FPGAs

A large share of today's HPC workloads is used for Ab-Initio Molecular Dynamics (AIMD) simulations, where the interatomic forces are computed on-the-fly by means of accurate electronic structure calculations. They are computationally intensive and thus constitute an interesting application class for energy-efficient hardware accelerators such as FPGAs. In this paper, we investigate the potential of offloading 3D Fast Fourier Transformations (FFTs) as a critical routine of plane-wave-based electronic structure calculations to FPGA and in conjunction demonstrate the tolerance of these simulations to lower precision computations.

==> abbreviations.tex <==
\begin{acronym}
\acro{MD}{Molecular Dynamics}
\acro{AIMD}{Ab-Initio Molecular Dynamics}
\acro{FPGA}{Field Programmable Gate Array}
\acro{HPC}{High Performance Computing}

\acro{3d FFT}{three-dimensional Fast Fourier Transformation}
\acro{1d FFT}{one-dimensional Fast Fourier Transformation}
\acro{FFT}{Fast Fourier Transformation}
\acro{HPCC}{HPC Challenge}
\acro{OpenCL}{Open Computing Language}
\acro{GPU}{Graphics Processing Unit}
\acro{FLOPS}{Floating Point Operations per Second}
\acro{HDL}{Hardware Description Language}
\acro{AC}{Approximate Computing}
\acro{DSP}{digital signal processing}
\end{acronym}
